A First Look at On-device Models in iOS Apps

Powered by the rising popularity of deep learning techniques on smartphones, on-device deep learning models are being used in vital fields like finance, social media, and driving assistance. Because of the transparency of the Android platform and the on-device models inside, on-device models on Android smartphones have been proven to be extremely vulnerable. However, due to the challenge in accessing and analysing iOS app files, despite iOS being a mobile platform as popular as Android, there are no relevant works on on-device models in iOS apps. Since the functionalities of the same app on Android and iOS platforms are similar, the same vulnerabilities may exist on both platforms. In this paper, we present the first empirical study about on-device models in iOS apps, including their adoption of deep learning frameworks, structure, functionality, and potential security issues. We study why current developers use different on-device models for one app between iOS and Android. We propose a more general attack against white-box models that does not rely on pre-trained models and a new adversarial attack approach based on our findings to target iOS's gray-box on-device models. Our results show the effectiveness of our approaches. Finally, we successfully exploit the vulnerabilities of on-device models to attack real-world iOS apps.

==> sections/background.tex <==
\section{background}

==> tables/_old_tab_framework.tex <==
\begin{table*}[t]
\begin{adjustbox}{width=\textwidth,center}
\centering
\small
\begin{tabular}{|l|c|c|c|c|c|c|}
\hline
\textbf{Framework} & \textbf{Owner} & \textbf{Supported Mobile Platform} &
\textbf{Mobile API} & \textbf{Is Open-source} & \textbf{Supported Model Format} & \textbf{Support Training} \\ \hline


ONNX~\cite{TensorFlow} & Google & Android CPU, GPU \& iOS CPU, GPU & Java, C, C++, OC & \cmark & Protobuf (\emph{.pb, .onnx}), Numpy (\emph{.npz}) & \cmark\\ \hline

TensorFlow~\cite{TensorFlow} & Google & / & / & \cmark & ProtoBuf (\emph{.pb, .pbtxt}), hdf5 (\emph{.h5}), json, YAML & \cmark\\ \hline

TF Lite~\cite{tflite} & Google & Android CPU, GPU \& iOS CPU, GPU & Java, Python, C++, OC, Swift & \cmark & FlatBuffers (\emph{.tflite}) & \cmark\\ \hline

Caffe~\cite{caffe} & Berkeley & Android CPU \& iOS CPU & C++ & \cmark & customized, json (\emph{.caffemodel, .prototxt}), json, YAML & \cmark\\ \hline

Caffe2~\cite{caffe2} & Facebook & Android CPU, GPU \& iOS CPU, GPU & C, C++ & \cmark & ProtoBuf (\emph{.pb}) & \cmark\\ \hline

MxNet~\cite{mxnet} & Apache Incubator & Android CPU \&  iOS CPU & C, C++ & \cmark & customized, json (\emph{.json, .params}) & \cmark\\ \hline

DeepLearning4J~\cite{dl4j}  & Skymind & Android CPU \& iOS CPU & Java & \cmark & customized (\emph{.zip}) & \cmark\\ \hline

ncnn~\cite{ncnn} & Tencent & Android CPU, GPU \& iOS CPU, GPU & C++ & \cmark & customized (\emph{.params, .bin}) & \xmark\\ \hline

OpenCV~\cite{opencv} & OpenCV Team & Android CPU, GPU \& iOS CPU & C, C++ & \cmark & TensorFlow, Caffe, Darknet, ONNX, Torch, PyTorch & \cmark\\ \hline

FeatherCNN~\cite{feathercnn} & Tencent & Android CPU \& iOS CPU & C++ & \cmark & customized (\emph{.feathermodel}) & \xmark\\ \hline

Paddle-Lite~\cite{mdl} & Baidu & Android CPU, GPU \& iOS CPU, GPU \& Kirin  NPU & Java, C++ & \cmark & parambase (\emph{.pdmodel, .pdparams, .pdopt}), TensorFlow, Caffe, ONNX, PyTorch & \xmark\\ \hline

% xNN~\cite{xnn} \zy{Inactive} & Alibaba & Android CPU, iOS CPU & unknown & \xmark & unknown & unknown\\ \hline

MNN~\cite{mnn} & Alibaba & Android CPU, GPU \& iOS CPU, GPU & Python, C++ & \cmark & TensorFlow, Caffe, Darknet, ONNX & \cmark\\ \hline

MACE~\cite{mace} & XiaoMi & ARM-based CPU, GPU, DSP\& Android CPU, GPU, DSP \& iOS CPU & C++ & \cmark & customized (\emph{.pb, .yml, .a}), TensorFlow, Caffe,  ONNX & \xmark\\ \hline

SNPE~\cite{snpe} & Qualcomm & Qualcomm CPU, GPU, DSP & Java, C++ & \xmark & customized (\emph{.dlc}) & \xmark\\ \hline

% CNNDroid~\cite{cnndroid} \zy{Inactive} & Oskouei et al. & Android CPU \& GPU & Java & \cmark & MessagePack (\emph{.model}) & \xmark\\ \hline

CoreML~\cite{coreml} & Apple & iOS CPU, GPU \& iPadOS CPU, GPU \& watchOS CPU, GPU & Swift, OC & \xmark & customized, ProtoBuf (\emph{.proto, .mlmodel}), TensorFlow, Caffe,  ONNX, PyTorch & \cmark\\ \hline

MindSpore~\cite{} & Huawei & Android CPU \& GPU & Java, C++ & \cmark & ProtoBuf (\emph{.proto, .ckpt}) & \cmark\\ \hline

PyTorch Mobile~\cite{pytorch} & Facebook & Android CPU, GPU \& iOS CPU, GPU & Java, OC, Swift & \cmark & customized, pickle (\emph{.ckpt, .pkl, .pt, .pth, .ptl}), ONNX & \xmark\\ \hline

Bender~\cite{} & Xmartlabs & iOS CPU, GPU & Swift & \cmark & Tensorflow & \xmark\\ \hline

Chainer~\cite{chainer} & Preferred Networks & / & / & \cmark & customized (\emph{.chainermodel}) & \cmark\\ \hline

CNTK~\cite{cntk} & Microsoft & / & / & \cmark & ProtoBuf (\emph{.proto}), ONNX & \cmark\\ \hline

DarkNet~\cite{cntk} & Joseph Redmon et al. & / & /   & \cmark & customized (\emph{.weights, .cfg}) & \cmark\\ \hline

PaddlePaddle~\cite{mdl} & Baidu & / & /   & \cmark &  parambase (\emph{.pdmodel, .pdparams, .pdopt}), TensorFlow, Caffe, ONNX, PyTorch & \cmark\\ \hline

% Torch~\cite{torch} \zy{Inactive} & Facebook & / & / & \cmark & customized (\emph{.dat}) & \cmark\\ \hline

PyTorch~\cite{pytorch} & Facebook & / & / & \cmark & customized, pickle (\emph{.ckpt, .pkl, .pt, .pth}), ONNX & \cmark\\ \hline

Deep Graph Library~\cite{} & Minjie Wang et al. & / & / & \cmark & TensorFlow, ONNX, PyTorch & \cmark\\ \hline

\end{tabular}
\end{adjustbox}
\caption{An overview of popular deep learning frameworks and their smartphone support at the time of writing (Sep. 2022).}
\label{tab:overview_of_frameworks}
\end{table*}

==> tables/fig_appRatings.tex <==
\begin{figure*}
	\centering
	\subfigure[App ratings of DL apps and non-DL apps]{
		\begin{minipage}[t]{0.49\linewidth}
			\centering
			\includegraphics[width=0.9\linewidth]{figures/ratings.png}\\
			\label{fig:ratings}
		\end{minipage}%
	}%
	\subfigure[Review numbers of DL apps and non-DL apps]{
		\begin{minipage}[t]{0.49\linewidth}
			\centering
			\includegraphics[width=0.9\linewidth]{figures/reviews.png}\\
			\label{fig:reviews}
		\end{minipage}%
	}%
	\vspace{-4mm}
	\caption{Analysis of apps with on-device models}
	\label{fig:appComparision}
\end{figure*}

==> tables/modelChange.tex <==



\begin{table*}[!ht]
    \centering
    \caption{Details of Android version apps}
    \begin{tabular}{|l|l|l|l|l|}
    \hline
        \textbf{App} & \textbf{Models on iOS app} & \textbf{Model function} & \textbf{Retain feature} & \textbf{Alternative methods} \\ \hline
        Strike: Bitcoin \& Payments & inference\_graph.tflite & object detection & No & remove features \\ \hline
        Hair Color Changer & hair\_segmentation.tflite & hair segmentation & Yes & on cloud \\ \hline
        Homebase Employee Scheduling & SSDOcr.mlmodelc & OCR text detection & Yes & unknown \\ \hline
        I am - Daily Affirmations & IAMRecommender.mlmodelc & tips recommendation & Yes & on cloud \\ \hline
        AfterShip Package Tracker & SSDOcr.mlmodelc & OCR text detection & No & remove features \\ \hline
        TickPick: No Fee Tickets & SSDOcr.mlmodelc & OCR text detection & Yes & unknown \\ \hline
        \multirow{2}*{adidas CONFIRMED} & FindFour.mlmodelc & object detection & \multirow{2}*{No} & \multirow{2}*{remove features} \\ 
        ~ & FourRecognize.mlmodelc & object detection & ~ & ~ \\ \hline
        \multirow{7}*{EnhanceFox - AI Photo Enhancer} & 73f89699081852c8.mlmodelc & \multirow{7}*{photo enhancement} & \multirow{7}*{yes} & \multirow{7}*{model compress} \\
        ~ & EVBodyML100S16FP16.mlmodelc & ~ & ~ & ~ \\ 
        ~ & facesr\_380000\_pt.mlmodelc & ~ & ~ & ~ \\ 
        ~ & RealESRGANv2-animevideo-xsx4.mlmodelc & ~ & ~ & ~ \\ 
        ~ & waifu2x\_upconv7\_anime\_0\_sim.mlmodelc & ~ & ~ & ~ \\ 
        ~ & waifu2x\_upconv7\_anime\_2\_sim.mlmodelc & ~ & ~ & ~ \\ 
        ~ & waifu2x\_upconv7\_anime\_3\_sim.mlmodelc & ~ & ~ & ~ \\ 
        \hline
    \end{tabular}
    \label{tab:modelChange}
\end{table*}

==> tables/tab_attackResults.tex <==


\begin{table*}[htbp]
  \centering
  \caption{Attack Results}
    \begin{adjustbox}{width=0.7\textwidth,center}
\begin{tabular}{|cc|cccccccccc|c|} 
\noalign{\hrule height 1pt}
Attack                      & Epsilon & M1   & M2   & M3   & M4   & M5   & M6   & M7   & M8   & M9   & M10  & Average  \\ 
\noalign{\hrule height 1pt}
Pointwise Attack            & 3.5     & 0.6  & 0.6  & 0.5  & 0.7  & 0.7  & 0.7  & 0.8  & 0.6  & 0.8  & 0.7  & 0.67     \\
Boundary Attack             & 5.5     & 0.5  & 0.7  & 0.8  & 0.7  & 0.6  & 0.8  & 0.5  & 0.6  & 0.8  & 0.8  & 0.68     \\
DDN Attack                  & 0.8     & 0.8  & 0.4  & 0.6  & 0.7  & 0.6  & 0.7  & 0.7  & 0.7  & 0.8  & 0.5  & 0.65     \\
DeepFool Attack             & 1.7     & 0.5  & 0.6  & 0.6  & 0.9  & 0.8  & 0.8  & 0.4  & 0.7  & 0.9  & 0.5  & 0.67     \\
FGSM                        & 0.02    & 0.6  & 0.7  & 0.8  & 0.7  & 0.7  & 0.6  & 0.5  & 0.7  & 0.8  & 0.7  & 0.68     \\
BIM                         & 2.5     & 0.6  & 0.6  & 0.9  & 0.5  & 0.2  & 0.8  & 0.7  & 0.8  & 0.9  & 0.6  & 0.66     \\
PGD                         & 8       & 0.5  & 0.5  & 0.7  & 0.8  & 0.5  & 0.5  & 0.7  & 0.8  & 0.6  & 0.7  & 0.63     \\
C\&W Attack                 & 0.6     & 0.7  & 0.6  & 0.5  & 0.8  & 0.5  & 0.7  & 0.5  & 0.6  & 0.9  & 0.6  & 0.64     \\
Newton Fool Attack          & 9.5     & 0.6  & 0.7  & 0.7  & 0.7  & 0.8  & 0.7  & 0.6  & 0.7  & 0.8  & 0.7  & 0.70     \\
Clipping-Aware Noise Attack & 20      & 0.8  & 0.9  & 0.9  & 0.8  & 0.9  & 0.8  & 0.8  & 0.9  & 0.8  & 0.9  & \textbf{0.85}     \\ 
\noalign{\hrule height 1pt}
Average (Models)            &         & 0.62 & 0.63 & 0.70 & 0.73 & 0.73 & 0.71 & 0.62 & 0.71 & \textbf{0.81} & 0.67 & 0.68     \\
\noalign{\hrule height 1pt}
\end{tabular}
    \end{adjustbox}
  \label{tab:results}%
\end{table*}%

==> tables/tab_attackResults2.tex <==
\begin{table*}[htbp]
  \centering
  \caption{Attack results of Core ML models on iOS and their counterparts on Android}
  \vspace{-4mm}
    \begin{adjustbox}{width=\textwidth,center}
    \begin{tabular}{|cc|cc|cc|cc|cc|cc|cc|cc|cc|cc|cc|cc|}
    \noalign{\hrule height 1pt}
    \textbf{Attack} & \textbf{Epsilon} & \multicolumn{2}{c|}{\textbf{M1}} & \multicolumn{2}{c|}{\textbf{M2}} & \multicolumn{2}{c|}{\textbf{M3}} & \multicolumn{2}{c|}{\textbf{M4}} & \multicolumn{2}{c|}{\textbf{M5}} & \multicolumn{2}{c|}{\textbf{M6}} & \multicolumn{2}{c|}{\textbf{M7}} & \multicolumn{2}{c|}{\textbf{M8}} & \multicolumn{2}{c|}{\textbf{M9}} & \multicolumn{2}{c|}{\textbf{M10}} & \multicolumn{2}{c|}{\textbf{Average}} \\
    \noalign{\hrule height 1pt}
     & & \textbf{A} & \textbf{I}  &\textbf{A} & \textbf{I} & \textbf{A} & \textbf{I} & \textbf{A} & \textbf{I} & \textbf{A} & \textbf{I} & \textbf{A} & \textbf{I} & \textbf{A} & \textbf{I} & \textbf{A} & \textbf{I} & \textbf{A} & \textbf{I} & \textbf{A} & \textbf{I} & \textbf{A} & \textbf{I} \\
    
    \hline
    
    Pointwise Attack & 3.5     & 0.6  & 0.6     & 0.6  & 0.6     & 0.6  & 0.5     & 0.7  & 0.7     & 0.8  & 0.7     & 0.7  & 0.7     & 0.8  & 0.8     & 0.6  & 0.6     & 0.8  & 0.8     & 0.8  & 0.7     & 0.7  & 0.67 \\
    
    Boundary Attack & 5.5     & 0.5  & 0.5    & 0.7  & 0.7    & 0.8  & 0.8    & 0.7  & 0.7    & 0.8  & 0.6   & 0.8  & 0.8    & 0.5  & 0.5    & 0.6  & 0.6   & 0.8  & 0.8    & 0.8  & 0.8    & 0.7  & 0.68\\
    
    DDN Attack & 0.8   & 0.8 & 0.8   & 0.4 & 0.4     & 0.7 & 0.6     & 0.7 & 0.7    & 0.6 & 0.6    & 0.7 & 0.7   & 0.7 & 0.7     & 0.7 & 0.7     & 0.8 & 0.8    & 0.7 & 0.5   & 0.68  & 0.65\\
    
    DeepFool Attack & 1.7   & 0.5 & 0.5   & 0.6 & 0.6     & 0.6 & 0.6     & 0.9 & 0.9    & 0.8 & 0.8    & 0.8 & 0.8   & 0.4 & 0.4     & 0.7 & 0.7     & 0.9 & 0.9    & 0.5 & 0.5   & 0.67  & 0.67 \\
    
    FGSM  & 0.02  & 0.6 & 0.6   & 0.7 & 0.7    & 0.8 & 0.8     & 0.7 & 0.7    & 0.7 & 0.7    & 0.6 & 0.6   & 0.5 & 0.5     & 0.7  & 0.7     & 0.8 & 0.8    & 0.8 & 0.7  & 0.69  & 0.68\\
    
    BIM & 2.5     & 0.6 & 0.6   & 0.6 & 0.6     & 0.9 & 0.9     & 0.5 & 0.5    & 0.2 & 0.2    & 0.8 & 0.8   & 0.7 & 0.7     & 0.8 & 0.8     & 0.9 & 0.9    & 0.8 & 0.6  & 0.64  & 0.62\\
    
    PGD & 8    & 0.5 & 0.5   & 0.5 & 0.5     & 0.9 & 0.8     & 0.8 & 0.8    & 0.5 & 0.5    & 0.5 & 0.5   & 0.7 & 0.7     & 0.8 & 0.8     & 0.6 & 0.6    & 0.7 & 0.7  & 0.65  & 0.64\\
    
    C\&W Attack & 0.6  & 0.7 & 0.7   & 0.6 & 0.6     & 0.5 & 0.5     & 0.8 & 0.8    & 0.6 & 0.5    & 0.7 & 0.7   & 0.5 & 0.5     & 0.6 & 0.6     & 0.9 & 0.9    & 0.6 & 0.6  & 0.65  & 0.64\\
    
    Newton Fool Attack & 9.5    & 0.6 & 0.6   & 0.7 & 0.7     & 0.7 & 0.7     & 0.7 & 0.6   & 0.8 & 0.8    & 0.7 & 0.7   & 0.6 & 0.6     & 0.7 & 0.7     & 0.8 & 0.8    & 0.7 & 0.7  & 0.7  & 0.69\\
    
    CAN Attack & 20    & 0.8 & 0.8   & 0.9 & 0.9     & 0.9 & 0.9     & 0.8 & 0.8    & 0.9 & 0.9     & 0.8 & 0.8   & 0.8 & 0.8     & 0.9 & 0.9     & 0.8 & 0.8    & 0.9 & 0.9  & \textbf{0.85}  & \textbf{0.85}\\
    \noalign{\hrule height 1pt}
    Average (Models) &   ~    & 0.62 & 0.62   & 0.63 & 0.63     & 0.7 & 0.67     & 0.73 & 0.72    & 0.73 & 0.71   & 0.71 & 0.71   & 0.62 & 0.62     & 0.71 & 0.71    & \textbf{0.81} & \textbf{0.81}    & 0.67 & 0.61  & 0.758  & 0.747 \\
    \noalign{\hrule height 1pt}
    \end{tabular}%
    \end{adjustbox}
  \label{tab:results}%
  
\end{table*}%


==> tables/tab_modelUsage.tex <==



\begin{table}[!ht]
    \caption{The usage of on-device models in iOS apps}
    \vspace{-4mm}
\begin{adjustbox}{width=0.3\textwidth, center}
    \centering
    \begin{tabular}{|c|c|c|}
        \noalign{\hrule height 1pt}
        \textbf{Field} & \textbf{Usage} & \textbf{Count} \\
        
        \noalign{\hrule height 1pt}
        
        \multirow{8}*{CV: 332}  & Photo beauty & 68 \\ 
        
        ~ & Object detection & 48 \\ 
        ~ & Image classification & 46 \\ 
        ~ & Face detection & 39 \\ 
        ~ & Image segmentation & 37 \\ 
        ~ & OCR Text recognition & 36 \\
        ~ & Augmented reality & 36 \\ 
        ~ &  Barcode scanning & 22 \\ 
        
        \hline
        
        \multirow{3}*{NLP: 23} & Language identification & 20 \\ 
        
        ~ & Smart reply & 2 \\
        
        ~ & Translation & 1 \\ \hline
        
        Audio: 10 & Sound recognition & 10 \\ \hline
        
        \multirow{5}*{Other: 55} & Recommendation & 17 \\
        
        ~ & Unknown & 15 \\
        
        ~ & Movement tracking & 13 \\
        
        ~ & Video segment & 5 \\
        
        ~ & Gesture recognition & 5 \\
        \noalign{\hrule height 1pt}
    \end{tabular}
\end{adjustbox}
    \label{tab:modelUsage}
    \vspace{-4mm}
\end{table}
